Magnitude-aware Probabilistic Speaker Embeddings

Recently, hyperspherical embeddings have established themselves as a dominant technique for face and voice recognition. Specifically, Euclidean space vector embeddings are learned to encode person-specific information in their direction while ignoring the magnitude. However, recent studies have shown that the magnitudes of the embeddings extracted by deep neural networks may indicate the quality of the corresponding inputs. This paper explores the properties of the magnitudes of the embeddings related to quality assessment and out-of-distribution detection. We propose a new probabilistic speaker embedding extractor using the information encoded in the embedding magnitude and leverage it in the speaker verification pipeline. We also propose several quality-aware diarization methods and incorporate the magnitudes in those. Our results indicate significant improvements over magnitude-agnostic baselines both in speaker verification and diarization tasks.

==> diarization/diarization.tex <==
\section{Speaker diarization}

% Also, we propose a two-stage speaker diarization algorithm which uses the most reliable segments to correctly determine initial clusters and their number followed by subsequent/label refinement. 


%We also explored the impact of Norm-Aware approaches in the Speaker Diarization task. 
%(todo: rewrite intro here)

%In this section we show how the magnitude-aware representation can improve speaker diarization performance
This section presents how to improve the speaker diarization performance by introducing a quality assessment into the processing pipeline. Thus, we propose the following two-stage diarization method. 
The first stage filters out the less reliable segments and finds initial clusters within the remaining segments.
The second stage uses all available segments and refines their labels based on the number of clusters estimated in the first stage. Additionally, we implemented the quality propagation into the VBx system (todo: link) and applied the two-stage diarization method to the VBx system.

%selects a subset of high quality segments, which is used to find initial labels.

%could be chosen by sorting magnitudes, and determine clusters amount using only selected segments. 


%consists of agglomerative clustering algorithm with the predefined (in the first stage) number of clusters. 



\subsection{Experiment Setup}

We conducted the experiments using the popular AMI corpus \cite{ami_corpus} and VOXCONVERSE (todo: link). 
%We use the XXX split 
We followed the development/evaluation split for AMI corpus from the official website \footnote{\scriptsize \url{https://groups.inf.ed.ac.uk/ami/corpus/datasets.shtml}} and for VOXCONVERSE we used dev v0.0.1/eval v0.0.2 sets from the \footnote{\scriptsize \url{https://github.com/joonson/voxconverse}}, where the development sets is used only for tuning the parameters of the clustering algorithm. That is, we used the same embeddings extractors as described in the previous section without fine-tuning on the AMI or VOXCONVERSE data.

% %\textbf{Data}. 
% %We use 
% We randomly selected 10 audio files for hyperparameters tuning and 5 audio files for evaluation from the AMI dataset (todo: link)
% The development part is used for tuning hyperparametrs of clustering algorithms.

% %\textbf{Training details}. 
% We trained embedders on the development part of the VoxCeleb2 dataset (Speaker Verification task). Detailed training recipe was described in section \ref{subsec:speaker_verification_training_recipe}. We didn't finetune embedders on any other datasets.

% About DER and JER
We used a simple speaker diarization pipeline including the following steps: voice activity detection (VAD) (todo: link to pyannote), overlapped speech detection (OSD) (todo: link to pyannote), fixed-length segmentation, clustering and resegmentation (todo: link to pyannote). 
We extracted embeddings from segments of length $1.5$ sec with $0.75$ overlap within the boundaries computed by VAD. 
%We extracted embeddings from segments of length $1.5$ sec shifted by $1.5$ sec within the boundaries computed by VAD. 
These embeddings were further clustered using one of the algorithms described below. Thereafter, we reassign labels for segments with overlaps detected by OSD module. We used simple heuristic: we assign two closest speakers to every segment marked by OSD.

\textbf{Algorithm "AHC"} We applied the agglomerative hierarchical clustering (AHC) algorithm described in \cite{landini2020bayesian}. The stopping threshold was tuned on the development set. We chose this algorithm as the baseline in the experiments.

\textbf{Algorithm "VB"} We implemented VBHMM diarization (aka VBx) proposed in \cite{landini2020bayesian}.

\textbf{Algorithm "VB\_UP"} We implemented uncertainty propagation into the BHMM backend using reciprocals for magnitudes as uncerainties. % (todo: expand description it)

The proposed two-stage algorithm sorts embeddings magnitudes and divides embeddings into two subsets based on the percentile tuned on the development set. Then, the first stage applies a general clustering algorithm with an unknown number of clusters (AHC/VBx in our case) to the set formed from embeddings with larger magnitudes. Intuitively, this should provide a better estimate for the number of clusters and their locations than one-stage algorithms. The resulting labels were used as input to the second stage of the algorithm, which has three possible implementations.

\textbf{Algorithm 2.1.} We computed the average embeddings (centroids) within each cluster found in the first stage and assigned the remaining embeddings to the closest centroid using similarity function.

\textbf{Algorithm 2.2.}  We applied a clustering algorithm with a fixed number of clusters (estimated in the first stage) to \textit{all} embeddings.

\textbf{Algorithm 2.3.} 
We applied a clustering algorithm with a fixed number of clusters to the \textit{remaining} embeddings.

We indicate these algorithms as a postfix to the clustering algorithm name. For instance, "VB\_UP (2.1)" means that we applied the VBx diarization with uncertainty propagation to the subset of embeddings with the largest magnitudes (by percentile tuned on the development set) and after we assigned the unsettled embeddings to the closest centroids.

To solve the label ambiguity problem in (2.3) algorithm, we computed the centroids of the clusters from the first stage and assigned the remaining embeddings to the closest centroid by cosine similarity. Finally, we found the dominating labels within each cluster found in the second stage and assigned this label to all the embeddings within this cluster.

In our experiments provided in the Table \ref{tab:two_stage_comparison}, we found that (2.1) provides slightly better results than (2.2) and (2.3). Therefore, we report the results only for (2.1). % (todo: provide experimental results)
%We used AHC from \cite{scikit-learn}
%in the second stage of Algorithm 2.2 and 2.3. %(todo: describe it in VBx case)

\subsection{Evaluation results}
We report the results using the Diarization error rate (DER) \cite{DER_explained} and Jaccard error rate (JER) \cite{DIHARD-2} metrics. Following common practice, we did not use the forgiveness collar. In addition, the speaker overlap regions were included during scoring at the evaluation stage. We followed these evaluation parameters in all tables with results except \ref{} (todo: link to the table BUT-Like).
 
\setlength{\tabcolsep}{3.0pt}   % space between columns


% todo: move this table to the appendix
\begin{table}[h]
\centering
\begin{tabular}{lcc}
\toprule
\multicolumn{1}{c}{\textbf{Clustering Algorithm}} & \textbf{DER, \%} & \textbf{JER, \%} \\ \toprule
AHC                                               & 22.75            & 28.29            \\ \hline
AHC (2.1)                                         & \textbf{13.13}   & \textbf{23.62}   \\ \hline
AHC (2.2)                                         & 19.07            & 25.75            \\ \hline
AHC (2.3)                                         & 17.04            & 26.68            \\ \hline
\end{tabular}
\caption{Comparison of two-stage clustering algorithms based on ResNet-MagFace embeddings extractor and AHC clustering algorithm. The evaluation was performed on the AMI Headset Mix channel without any forgiveness collar and }
% Results are presented for the AMI dataset.
\label{tab:two_stage_comparison}
\end{table}


\begin{table}[!h]
\begin{tabular}{llllll}
\hline
\multicolumn{2}{c}{\textbf{Setup}}   & \multicolumn{1}{c}{\textbf{Clustering}} & \multicolumn{1}{c}{\textbf{OSD}} & \multicolumn{1}{c}{\textbf{DER, \%}} & \textbf{JER, \%} \\ \hline
collar & \multicolumn{1}{c}{overlap} & \multicolumn{1}{c}{}                     & \multicolumn{1}{c}{}             & \multicolumn{1}{c}{}                 &                  \\ \hline
0.25   & No                          & \multirow{3}{*}{AHC}                     & \multirow{3}{*}{No}              & 6.89                                 & \multirow{3}{*}{32.59}            \\
0.25   & Yes                         &                                          &                                  & 16.58                                &             \\
0      & Yes                         &                                          &                                  & 27.27                                &             \\ \hline
0.25   & No                          & \multirow{3}{*}{AHC (2.1)}                 & \multirow{3}{*}{No}              & 2.76                                 & \multirow{3}{*}{28.12}            \\
0.25   & Yes                         &                                          &                                  & 11.74                                &             \\
0      & Yes                         &                                          &                                  & 20.66                                &             \\ \hline
0.25   & No                          & \multirow{3}{*}{AHC}                     & \multirow{3}{*}{Yes}             & 6.89                                 & \multirow{3}{*}{28.29}            \\
0.25   & Yes                         &                                          &                                  & 13.91                                &             \\
0      & Yes                         &                                          &                                  & 22.75                                &             \\ \hline
0.25   & No                          & \multirow{3}{*}{AHC (2.1)}                 & \multirow{3}{*}{Yes}             & 2.76                                 & \multirow{3}{*}{23.62}            \\
0.25   & Yes                         &                                          &                                  & 7.07                                 &             \\
0      & Yes                         &                                          &                                  & 13.13                                &             \\ \hline
\end{tabular}
\caption{Comparison of speaker diarization methods based on different clustering algorithms with and without Overlapped Speech Detection module. The evaluation was performed on the AMI Headset Mix channel.}
% Results are presented for the AMI dataset.
\label{tab:diar_comparison_AMI}
\end{table}


\begin{table}[!h]
\begin{tabular}{llllll}
\hline
\multicolumn{2}{c}{\textbf{Setup}}   & \multicolumn{1}{c}{\textbf{Clustering}} & \multicolumn{1}{c}{\textbf{OSD}} & \multicolumn{1}{c}{\textbf{DER, \%}} & \textbf{JER, \%} \\ \hline
collar & \multicolumn{1}{c}{overlap} & \multicolumn{1}{c}{}                    & \multicolumn{1}{c}{}             & \multicolumn{1}{c}{}                 &                  \\ \hline
0.25   & No                          & \multirow{3}{*}{AHC}                    & \multirow{3}{*}{No}              & 5.18                                 & \multirow{3}{*}{23.71}            \\
0.25   & Yes                         &                                         &                                  & 7.06                                 &                  \\
0      & Yes                         &                                         &                                  & 11.76                                &                  \\ \hline
0.25   & No                          & \multirow{3}{*}{AHC (2.1)}                & \multirow{3}{*}{No}              & 4.2                                  & \multirow{3}{*}{30.61}            \\
0.25   & Yes                         &                                         &                                  & 7.21                                 &             \\
0      & Yes                         &                                         &                                  & 12.3                                 &             \\ \hline
0.25   & No                          & \multirow{3}{*}{AHC}                    & \multirow{3}{*}{Yes}             & 5.2                                  & \multirow{3}{*}{22.25}            \\
0.25   & Yes                         &                                         &                                  & 6.32                                 &             \\
0      & Yes                         &                                         &                                  & 10.41                                &             \\ \hline
0.25   & No                          & \multirow{3}{*}{AHC (2.1)}                & \multirow{3}{*}{Yes}             & 4.26                                 & \multirow{3}{*}{28.71}            \\
0.25   & Yes                         &                                         &                                  & 5.53                                 &             \\
0      & Yes                         &                                         &                                  & 9.06                                 &             \\ \hline
\end{tabular}
\caption{Comparison of speaker diarization methods based on different clustering algorithms with and without Overlapped Speech Detection module. The evaluation was performed on the VOXCONVERSE test v0.0.2.}
% Results are presented for the AMI dataset.
\label{tab:diar_comparison_VOXCONVERSE}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[!h]
% \footnotesize
% \begin{tabular}{cccccc}
% \hline
% \textbf{Dataset}                                  & \textbf{VAD, OSD}       & \textbf{Clustering}                           & \textbf{Reseg.} & \textbf{DER, \%} & \textbf{JER, \%} \\ \hline
% \multicolumn{1}{c|}{\multirow{8}{*}{\rotatebox[origin=c]{90}{AMI}}}         & \multirow{4}{*}{oracle} & \multicolumn{1}{|c|}{\multirow{2}{*}{AHC}}     & -               & 22.75            & 28.29            \\ \cline{4-6} 
% \multicolumn{1}{c|}{}                             &                         & \multicolumn{1}{|c|}{}                         & +               & 25.9             & 30.8             \\ \cline{3-6} 
% \multicolumn{1}{c|}{}                             &                         & \multicolumn{1}{|c|}{\multirow{2}{*}{AHC\_UP}} & -               & 13.13            & 23.62            \\ \cline{4-6} 
% \multicolumn{1}{c|}{}                             &                         & \multicolumn{1}{|c|}{}                         & +               & 22.29            & 28.58            \\ \cline{2-6} 
% \multicolumn{1}{c|}{}                             & \multirow{4}{*}{system} & \multicolumn{1}{|c|}{\multirow{2}{*}{AHC}}     & -               & 28.39            & 31.95            \\ \cline{4-6} 
% \multicolumn{1}{c|}{}                             &                         & \multicolumn{1}{|c|}{}                         & +               & 25.23            & 30.28            \\ \cline{3-6} 
% \multicolumn{1}{c|}{}                             &                         & \multicolumn{1}{|c|}{\multirow{2}{*}{AHC\_UP}} & -               & 24.2             & 29.41            \\ \cline{4-6} 
% \multicolumn{1}{c|}{}                             &                         & \multicolumn{1}{|c|}{}                         & +               & 23.14            & 29.19            \\ \hline
% \multicolumn{1}{c|}{\multirow{8}{*}{\rotatebox[origin=c]{90}{VOXCONVERSE}}} & \multirow{4}{*}{oracle} & \multicolumn{1}{|c|}{\multirow{2}{*}{AHC}}     & -               & 10.41            & 22.25            \\ \cline{4-6} 
% \multicolumn{1}{c|}{}                             &                         & \multicolumn{1}{|c|}{}                         & +               & 12.73            & 24.82            \\ \cline{3-6} 
% \multicolumn{1}{c|}{}                             &                         & \multicolumn{1}{|c|}{\multirow{2}{*}{AHC\_UP}} & -               & 9.06             & 28.71            \\ \cline{4-6} 
% \multicolumn{1}{c|}{}                             &                         & \multicolumn{1}{|c|}{}                         & +               & 12.67            & 30.11            \\ \cline{2-6} 
% \multicolumn{1}{c|}{}                             & \multirow{4}{*}{system} & \multicolumn{1}{|c|}{\multirow{2}{*}{AHC}}     & -               & 15.82            & 25.26            \\ \cline{4-6} 
% \multicolumn{1}{c|}{}                             &                         & \multicolumn{1}{|c|}{}                         & +               & 13.15            & 25.91            \\ \cline{3-6} 
% \multicolumn{1}{c|}{}                             &                         & \multicolumn{1}{|c|}{\multirow{2}{*}{AHC\_UP}} & -               & 12.98            & 28.91            \\ \cline{4-6} 
% \multicolumn{1}{c|}{}                             &                         & \multicolumn{1}{|c|}{}                         & +               & 11.42            & 27.65            \\ \hline
% \end{tabular}
% \caption{Comparison of speaker diarization methods based on different clustering algorithms with Oracle and System VAD and OSD modules, with and without resegmentation module. The evaluation was performed on the AMI Headset Mix channel and the VOXCONVERSE test v0.0.2. The magface model was used.} % todo change the last sentence
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!h]
\footnotesize
\begin{tabular}{ccccc}
\hline
\textbf{Dataset}                                   & \textbf{Model}               & \textbf{Clustering} & \textbf{DER, \%} & \textbf{JER, \%} \\ \hline
\multicolumn{1}{c|}{\multirow{12}{*}{\rotatebox[origin=c]{90}{AMI}}}         & \multirow{4}{*}{arcface}     & \multicolumn{1}{|c}{AHC}                 & 21.68            & 27.36            \\ \cline{3-5} 
\multicolumn{1}{c|}{}                              &                              & \multicolumn{1}{|c}{AHC (2)}             & 13.06            & 24.11            \\ \cline{3-5} 
\multicolumn{1}{c|}{}                              &                              & \multicolumn{1}{|c}{VB}                  & 20.13            & 27.86            \\ \cline{3-5} 
\multicolumn{1}{c|}{}                              &                              & \multicolumn{1}{|c}{VB\_UP (2)}          & 13.49            & 28.73            \\ \cline{2-5} 
\multicolumn{1}{c|}{}                              & \multirow{4}{*}{magface}     & \multicolumn{1}{|c}{AHC}                 & 22.75            & 28.29            \\ \cline{3-5} 
\multicolumn{1}{c|}{}                              &                              & \multicolumn{1}{|c}{AHC (2)}             & 13.13            & 23.62            \\ \cline{3-5} 
\multicolumn{1}{c|}{}                              &                              & \multicolumn{1}{|c}{VB}                  & 20.52            & 29.23            \\ \cline{3-5} 
\multicolumn{1}{c|}{}                              &                              & \multicolumn{1}{|c}{VB\_UP (2)}          & 13.02            & 26.22            \\ \cline{2-5} 
\multicolumn{1}{c|}{}                              & \multirow{4}{*}{magface big} & \multicolumn{1}{|c}{AHC}                 & 20.15            & 25.95            \\ \cline{3-5} 
\multicolumn{1}{c|}{}                              &                              & \multicolumn{1}{|c}{AHC (2)}             & 15.87            & 24.34            \\ \cline{3-5} 
\multicolumn{1}{c|}{}                              &                              & \multicolumn{1}{|c}{VB}                  & 20.38            & 27.69            \\ \cline{3-5} 
\multicolumn{1}{c|}{}                              &                              & \multicolumn{1}{|c}{VB\_UP (2)}          & 13.67            & 26.71            \\ \hline
\multicolumn{1}{c|}{\multirow{12}{*}{\rotatebox[origin=c]{90}{VOXCONVERSE}}} & \multirow{4}{*}{arcface}     & \multicolumn{1}{|c}{AHC}                 & 10.71            & 24.4             \\ \cline{3-5} 
\multicolumn{1}{c|}{}                              &                              & \multicolumn{1}{|c}{AHC (2)}            & 8.22             & 27.36            \\ \cline{3-5} 
\multicolumn{1}{c|}{}                              &                              & \multicolumn{1}{|c}{VB}                  & 10.33            & (JER PROB) \\ \cline{3-5} 
\multicolumn{1}{c|}{}                              &                              & \multicolumn{1}{|c}{VB\_UP (2)}          & (JER PROB)     & (JER PROB)     \\ \cline{2-5} 
\multicolumn{1}{c|}{}                              & \multirow{4}{*}{magface}     & \multicolumn{1}{|c}{AHC}                 & 10.41            & 22.25            \\ \cline{3-5} 
\multicolumn{1}{c|}{}                              &                              & \multicolumn{1}{|c}{AHC (2)}             & 7.67             & 27.74            \\ \cline{3-5} 
\multicolumn{1}{c|}{}                              &                              & \multicolumn{1}{|c}{VB}                  & (JER PROB)     & (JER PROB)     \\ \cline{3-5} 
\multicolumn{1}{c|}{}                              &                              & \multicolumn{1}{|c}{VB\_UP (2)}          & (JER PROB)     & (JER PROB)     \\ \cline{2-5} 
\multicolumn{1}{c|}{}                              & \multirow{4}{*}{magface big} & \multicolumn{1}{|c}{AHC}                 & 8.61             & 21.97            \\ \cline{3-5} 
\multicolumn{1}{c|}{}                              &                              & \multicolumn{1}{|c}{AHC (2)}             & 7.46             & 24.36            \\ \cline{3-5} 
\multicolumn{1}{c|}{}                              &                              & \multicolumn{1}{|c}{VB}                  & (JER PROB)     & (JER PROB)     \\ \cline{3-5} 
\multicolumn{1}{c|}{}                              &                              & \multicolumn{1}{|c}{VB\_UP (2)}          & (JER PROB)     & (JER PROB)     \\ \hline
\end{tabular}
\caption{Comparison of speaker diarization methods based on different clustering algorithms and different embedder models with Oracle VAD and OSD modules and without resegmentation module. The evaluation was performed on the AMI Headset Mix channel and the VOXCONVERSE test v0.0.2.}
\end{table}

% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table}[]
% \begin{tabular}{cccc}
% \hline
% \textbf{Dataset}                                  & \textbf{clustering\_type} & \textbf{DER}   & \textbf{JER}   \\ \hline
% \multicolumn{1}{c|}{\multirow{6}{*}{AMI}}         & AHC                       & 22.75          & 28.29          \\
% \multicolumn{1}{c|}{}                             & AHC (2)                   & 13.13          & \textbf{23.62} \\
% \multicolumn{1}{c|}{}                             & VB                        & 20.52          & 29.23          \\
% \multicolumn{1}{c|}{}                             & VB (2)                    & 15.34          & 26.05          \\
% \multicolumn{1}{c|}{}                             & VB\_UP                    & 17.86          & 27.11          \\
% \multicolumn{1}{c|}{}                             & VB\_UP (2)                & \textbf{13.02} & 26.22          \\ \hline
% \multicolumn{1}{c|}{\multirow{6}{*}{VOXCONVERSE}} & AHC                       & 10.41          & 22.25          \\
% \multicolumn{1}{c|}{}                             & AHC (2)                   & 7.67           & 27.74          \\
% \multicolumn{1}{c|}{}                             & VB                        & todo           & todo           \\
% \multicolumn{1}{c|}{}                             & VB (2)                    & todo           & todo           \\
% \multicolumn{1}{c|}{}                             & VB\_UP                    & todo           & todo           \\
% \multicolumn{1}{c|}{}                             & VB\_UP (2)                & todo           & todo           \\ \hline
% \end{tabular}
% \end{table}


% Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table}[]
% \begin{tabular}{ccccc}
% \hline
% \textbf{Dataset}                                  & \textbf{Clustering}                                & \textbf{Scoring} & \textbf{DER}   & \textbf{JER}   \\ \hline
% \multicolumn{1}{c|}{\multirow{4}{*}{AMI}}         & \multicolumn{1}{c|}{\multirow{2}{*}{AHC}}          & cos              & \textbf{22.75} & \textbf{28.29} \\
% \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                              & gme              & 25.66          & 29.77          \\ \cline{2-5} 
% \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{\multirow{2}{*}{AHC two step}} & cos              & 13.13          & \textbf{23.62} \\
% \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                              & gme              & \textbf{12.96} & 23.85          \\ \hline
% \multicolumn{1}{c|}{\multirow{4}{*}{VOXCONVERSE}} & \multicolumn{1}{c|}{\multirow{2}{*}{AHC}}          & cos              & \textbf{10.41} & \textbf{22.25} \\
% \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                              & gme              & 11.56          & 24.39          \\ \cline{2-5} 
% \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{\multirow{2}{*}{AHC two step}} & cos              & \textbf{7.67}  & 27.74          \\
% \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                              & gme              & 7.89           & \textbf{26.79} \\ \hline
% \end{tabular}
% \end{table}



First, two of the three variants of the proposed method significantly outperformed the baseline in the DER metric. For the magnitude-aware losses, we report the results only for Algorithm 2.1 because it performed the best.
The proposed method achieved at least a $25 \%$ relative reduction in DER among all compared losses. For instance, one of the highest relative reductions of approximately $47 \%$ (from $5.28 \%$ to $2.80 \%$) was obtained by MagFace (ArcFace, $\lambda_g=0.5$), which demonstrates the benefit of the presented quality-aware diarization method.

